Adapting to Mixing Time in Stochastic Optimization with Markovian Data

We consider stochastic optimization problems where data is drawn from a Markov chain. Existing methods for this setting crucially rely on knowing the mixing time of the chain, which in real-world applications is usually unknown. We propose the first optimization method that does not require the knowledge of the mixing time, yet obtains the optimal asymptotic convergence rate when applied to convex problems. We further show that our approach can be extended to: (i) finding stationary points in non-convex optimization with Markovian data, and (ii) obtaining better dependence on the mixing time in temporal difference (TD) learning; in both cases, our method is completely oblivious to the mixing time. Our method relies on a novel combination of multi-level Monte Carlo (MLMC) gradient estimation together with an adaptive learning method.

==> AC_response.tex <==
Dear area chair,

We are concerned that Reviewer #2 didn't understand major parts of our work -- he claims that our MLMC gradient estimation technique, which is a crucial ingredient in our scheme, is not necessary. Moreover, he questions the novelty of our approach, which is unanimously acknowledged by the other reviewers. 

We kindly ask the chair to discount Reviewer #2's evaluation. 

% Reviewer 3 gave a very negative review with very little actual content to support it. Some claims are completely vacuous, such as expecting our method to learn without relevant data (e.g., learn on semi-circle domain with only a few goals -- no method can do that without prior knowledge). Some illustrative claims are actually rigorously addressed in our theory (e.g., the example with multiple goals). Others are just nitpicks, such as our choice of data collection using RL agents, which we specifically claimed is used to ground our investigation in a simple and practical application.

% We kindly ask the reviewer to discount Reviewer 3's evaluation, and bring these issues to the attention of the other reviewers in the discussion. 

% Reviewer 6 gave a very positive view on the broad implications of our work, and we hope that the discussion will not dominated by nitpicks that are based on shallow understanding of the work by Reviewer 3.

